Boosting Search Engines with Interactive Agents

This paper presents first successful steps in designing search agents that learn meta-strategies for iterative query refinement in information-seeking tasks. Our approach uses machine reading to guide the selection of refinement terms from aggregated search results. Agents are then empowered with simple but effective search operators to exert fine-grained and transparent control over queries and search results. We develop a novel way of generating synthetic search sessions, which leverages the power of transformer-based language models through (self-)supervised learning. We also present a reinforcement learning agent with dynamically constrained actions that learns interactive search strategies from scratch. Our search agents obtain retrieval and answer quality performance comparable to recent neural methods, using only a traditional term-based BM25 ranking function and interpretable discrete reranking and filtering actions.

==> sections/2-search.tex <==
\section{Self-Supervised "Learning to Search"} 
\label{sect:learning-to-search}

It has been a powerful vision for more than 20 years to design search engines that are intuitive and simple to use. Despite their remarkable success, search engines are not perfect and may not yield the most relevant result(s) in one shot. This is particularly true for rare and intrinsically difficult queries, which may require interactive exploration by the user to be answered correctly and exhaustively.
Contextual query refinement is a common technique~\citep{jansen2009}, even among children~\citep{rutter-etal-2015}, used to improve search by combining evidence from previous results and background knowledge~\citep{huang2009}. Such refinements often rely on inspecting result snippets and titles or on skimming the content of top-ranked documents. This process is iterative and may be repeated to produce a sequence of queries $q_0, q_1,\dots, q_T$ until (optimistically) a satisfactory answer is found. It seems natural to mimic this interactive process by a search agent, which learns the basic step of generating a follow-up query from previous queries and their search results.  

Furthermore, it is noteworthy how power users apply dedicated search operators and sophisticated investigative strategies to solve deep search puzzles~\citep{joy-of-search}. In particular, unary operators 
offer a great deal of fine-grained control and transparency and as such are highly effective in expert hands. We concentrate on three operators: `+', which limits results to documents that contain a specific term, `-' which excludes results that contain the term, and `${\scriptstyle \wedge}_i$' which boosts a term weight in the BM25 score computation by a factor $i\in\mathbb{R}$. 
For instance -- see also Figure~\ref{fig:architecture} -- the query 'who won the us open', may lead to both tennis and golf-related results. An expert searcher who wanted to zero-in on the tennis intent could do so by excluding golf-related terms and boosting tennis-related ones.
As we show in this paper, these operators are also pivotal in designing interactive search agents.

\subsection{Result Aggregation for Contextual Refinement}
\label{sec:aggregation}
Web searchers expect the best answer to be among the top few hits on the first results page~\citep[\S 5]{hearst2009search} and pay marginal attention to the bottom half of the \emph{10 blue links}~\citep{granka2004, joachims2005,nielsen-pernice-2009,info-eye-tracking}. Likewise, a search agent considers only the top $k$ documents returned by the search engine at every step, where $k=5$. During a search session the agent maintains a list of the top-$k$ documents overall, which is returned at the end.

To aggregate results we use a machine reader (MR), e.g., cf. \citep{rajpurkar-etal-2016-squad}. %
Specifically, we use a DPR-like reader/passage scorer~\citep{dpr}, which builds upon a pre-trained BERT model. Beyond identifying the most promising answer span within each result document $d$, the system also estimates the probability of $d$ containing the (unspecified) answer $\text{P}(d \ni \text{\textsc{\small answer}}\,\vert\,q) \in [0;1]$. This probability can be viewed as a Passage Score (PS) that induces a calibrated ranking across all result documents within a session.

An observation representing the session at any given step is built by extracting a fixed-length
%
token window centered at the answer span predicted by the reader for each document. In addition, we include the document titles. Finally, the query tokens and refinements describing $q_t$ are also included. This leads to a segmented observation token sequence $o_t$ which is truncated to length $\le 512$ , a common input length for pre-trained transformer-based LMs (cf. Appendix \ref{sec:a-observations-details} for details, examples).
We then use BERT or T5 to produce an embedding $\mathbf s_t$ from which the search agent will generate the next query. If we denote the result set for $q_t$ by $\mathcal D_t$, then we get diagrammatically 
\begin{align}
\begin{bmatrix}
q_0,\dots,q_t
\\[0mm]
\text{\tiny search} \downarrow \text{\tiny engine}
\\[1mm]
\mathcal D_0, \dots, \mathcal D_t
\end{bmatrix}
\; 
\underbrace{\stackrel{\text{MR/PS}} \longmapsto  \; o_t}_{\text{observation}} \;\; \underbrace{\stackrel{\text{LM}}{\longmapsto} \; \mathbf s_t}_{\text{encoding}} \;\; \underbrace{\stackrel{\text{agent}}\longmapsto \; q_{t+1}}_{\text{generation}}
\end{align}
We focus on the case where $q_{t+1}$ is obtained from $q_t$ through augmentation. This may add a keyword $w \in \Sigma^{\text{\tiny idx}}$, where $\Sigma^{\text{\tiny idx}}$ is the  search index vocabulary, with the usual disjunctive search engine semantics or a structured search term formed by the use of unary operators (`+',`-',`$\scriptstyle\wedge$') and  fields.

\subsection{Rocchio Query Expansions}
\label{sec:rocchio}

In the absence of training sessions from human expert users, we propose to generate synthetic search sessions in a self-supervised manner, making use of a set of question-answer pairs $(q,a)$. 
%
We initialize $q_0{=}q$ and aim to find a sequence of refinements that make progress towards identifying documents containing the answer $a$, based on a designed scoring function (cf. \S\ref{sect:openqa-env}). A query is \textit{not} further refined, if either $t{=}20$ (maximal length) or if no score increasing refinement can be found. 

To create candidate refinements, we make use of the idea of relevance feedback as suggested in \citet{rocchio71relevance}.  An elementary refinement -- called a \textit{Rocchio expansion} -- then takes the form 
\begin{align}
q_{t+1} := q_t \; \Delta q_t, \Delta q_t := [+\vert-\vert\wedge_i \;\; \text{\textsc{\small Title}}\, \vert \, \text{\textsc{\small Content}} \,] %\vert \, \epsilon
\;\; w_t, w_t \in \Sigma_t :=\Sigma_t^{q} \cup \Sigma_t^\tau \cup \Sigma_t^{\alpha} \cup \Sigma_t^{\beta}
\end{align}
where $i$ is the boosting coefficient and $\Sigma_t$ refers to a set of terms accessible to the agent. By that we mean terms that occur in the top PS-ranked session documents. We use superscripts to refer to the vocabulary of the question ($q$), titles ($\tau$), answers ($\alpha$) or bodies ($\beta$) of documents in $o_t$. Note that adding terms $\not\in \Sigma_t$ would make refinements difficult to reproduce for an agent and thus would provide supervision of low utility.

An important aspect of creating sessions as described above has to do with the search complexity of finding optimal sequences of Rocchio expansions. We consider $q_* = q + a$ as the ``ideal'' query, whose results define the vocabulary $\Sigma_*$. For efficiency reasons, we further constrain the terms to be added via exact matches, term boosting or term exclusions by defining two constrained dictionaries
\begin{align}\label{eq:dictionaries}
\Sigma^{\uparrow}_t = \Sigma_t \cap \Sigma_*, \quad 
\Sigma^{\downarrow}_t = \Sigma_t - \Sigma_*\,.
\end{align}
During the search for a successful session, it is possible to upgrade accessible terms, $w_t$, to exact matches (`+'), or weight boosting (`$\scriptstyle\wedge$'), if they also occur in the ideal result set ($w_t\in\Sigma^{\uparrow}_t$); and to exclude accessible terms (`-') if they are not present in the ideal results ($w_t\in\Sigma^{\downarrow}_t$). We have found experimentally that this leads to a good trade-off between the quality of Rocchio expansions and the search effort to find them. The search for sequences of Rocchio expansions is done heuristically. More implementation details, pseudo-code illustrating the procedure and examples can be found in \S\ref{sec:experiments}, Appendix~\ref{rocchio-procedure}, and Appendix~\ref{sect:app-session-examples}.

\subsection{Self-Supervised T5 Agent}
\label{sec:t5agent}
We suggest to train a generative search agent in a supervised manner by making use of synthetic search sessions generated by Rocchio expansions. We use T5,  
a popular pretrained transformer encoder-decoder model. % which achieves state-of-the-art results on multiple NLU tasks.
As a search agent, T5 predicts a single new search expansion from an observed state. 
In the spirit of \emph{everything-is-string-prediction}, both state and expansions are represented as plain strings. See Appendix \ref{sec:a-observations-details} for a full example.

Our T5 agent is trained via Behavioral Cloning (BC)~\citep{Michie1990}. We treat each step in a Rocchio session as a single training example. As is common in sequence prediction tasks, we use the cross-entropy loss for optimization. BC is perhaps the simplest form of Imitation Learning (IL), and has been proven effective in a variety of application domains~\citep{sharma2018,rodriguez2019}. In our query refinement task, it allows to inherit the expressive power of the Rocchio query expansions and, differently from other IL approaches~\citep{ross11a,ho2016,Ding2020}, requires only \emph{offline} interactions with the search engine. Crucially, this enables scaling to the large action spaces and model sizes typical of recent LMs. Our T5 agent can also be described as a Decision Transformer with fixed max return~\citep{decisiontransformer}.
